Threshold UCT: Cost-Constrained Monte Carlo Tree Search with Pareto Curves

Constrained Markov decision processes (CMDPs), in which the agent optimizes expected payoffs while keeping the expected cost below a given threshold, are the leading framework for safe sequential decision making under stochastic uncertainty. Among algorithms for planning and learning in CMDPs, methods based on Monte Carlo tree search (MCTS) have particular importance due to their efficiency and extendibility to more complex frameworks (such as partially observable settings and games). However, current MCTS-based methods for CMDPs either struggle with finding safe (i.e., constraint-satisfying) policies, or are too conservative and do not find valuable policies. We introduce Threshold UCT (T-UCT), an online MCTS-based algorithm for CMDP planning. Unlike previous MCTS-based CMDP planners, T-UCT explicitly estimates Pareto curves of cost-utility trade-offs throughout the search tree, using these together with a novel action selection and threshold update rules to seek safe and valuable policies. Our experiments demonstrate that our approach significantly outperforms state-of-the-art methods from the literature.

==> tables/ccpomcp.tex <==
\small
\begin{tabular}{lrrrr}
    \toprule
     & \multicolumn{2}{c}{CMDP1} & \multicolumn{2}{c}{CMDP2} \\
     & $\payoff$ & $\acost$ & $\payoff$ & $\acost$ \\
    \midrule
    T-UCT (ours) & 11.32 & 0.50 & 3.94 & 0.10 \\
    RAMCP & 9.41 & 0.52 & 3.43 & 0.16 \\
    CC-POMCP & 4.35 & 0.31 & 2.22 & 0.12 \\
    \bottomrule
    \end{tabular}
    

==> tables/gridworld_results.tex <==
\newcommand{\lopt}[1]{\textbf{#1}}

\small
\begin{tabular}{p{0.15cm}p{0.25cm}rp{0.22cm}p{1.4cm}p{0.22cm}p{1.5cm}r}
    \toprule
    & $\tps(\text{ms})$ & $\explconst$ & $\esat$ & & $\csat$ & & $\ncv$ \\
    \midrule
    
    
    \multirow{9}{*}{\rotatebox{90}{T-UCT (ours)}} & \multirow{3}{*}{1} & 0.1 & \lopt{160} &  ($122 \mid 38$) & \lopt{275} &  ($177 \mid 98$) & \lopt{0.60} \\
     &  & 5.0 & 140 &  ($110 \mid 30$) & 255 &  ($175 \mid 80$) & 0.58 \\
     &  & 20.0 & 137 &  ($112 \mid 25$) & 244 &  ($167 \mid 77$) & 0.54 \\
    \cline{2-8}
     & \multirow{3}{*}{2} & 0.1 & \lopt{203} &  ($142 \mid 61$) & \lopt{338} &  ($189 \mid 149$) & \lopt{0.72} \\
     &  & 5.0 & 193 &  ($131 \mid 62$) & 329 &  ($193 \mid 136$) & 0.71 \\
     &  & 20.0 & 176 &  ($129 \mid 47$) & 314 &  ($190 \mid 124$) & 0.68 \\
    \cline{2-8}
     & \multirow{3}{*}{5} & 0.1 & 241 &  ($145 \mid 96$) & 369 &  ($194 \mid 175$) & 0.76 \\
     &  & 5.0 & \lopt{245} &  ($156 \mid 89$) & \lopt{373} &  ($197 \mid 176$) & \lopt{0.79} \\
     &  & 20.0 & 216 &  ($136 \mid 80$) & 361 &  ($195 \mid 166$) & 0.74 \\
    \cline{1-8}
    \multirow{9}{*}{\rotatebox{90}{RAMCP}} & \multirow{3}{*}{1} & 0.1 & 35 &  ($24 \mid 11$) & 69 &  ($48 \mid 21$) & 0.18 \\
     &  & 5.0 & \lopt{159} &  ($124 \mid 35$) & \lopt{255} &  ($182 \mid 73$) & \lopt{0.58} \\
     &  & 20.0 & 143 &  ($106 \mid 37$) & 241 &  ($173 \mid 68$) & 0.54 \\
    \cline{2-8}
     & \multirow{3}{*}{2} & 0.1 & 36 &  ($22 \mid 14$) & 78 &  ($48 \mid 30$) & 0.20 \\
     &  & 5.0 & \lopt{178} &  ($130 \mid 48$) & \lopt{299} &  ($196 \mid 103$) & \lopt{0.65} \\
     &  & 20.0 & 164 &  ($123 \mid 41$) & 277 &  ($183 \mid 94$) & 0.59 \\
    \cline{2-8}
     & \multirow{3}{*}{5} & 0.1 & 48 &  ($27 \mid 21$) & 91 &  ($51 \mid 40$) & 0.25 \\
     &  & 5.0 & \lopt{215} &  ($139 \mid 76$) & \lopt{326} &  ($195 \mid 131$) & \lopt{0.71} \\
     &  & 20.0 & 203 &  ($141 \mid 62$) & 305 &  ($196 \mid 109$) & 0.65 \\
     \cline{1-8}
     \multirow{9}{*}{\rotatebox{90}{CC-POMCP}} & \multirow{3}{*}{1} & 0.1 & 123 &  ($97 \mid 26$) & 146 &  ($115 \mid 31$) & \lopt{0.18} \\
     &  & 5.0 & \lopt{132} &  ($101 \mid 31$) & \lopt{160} &  ($119 \mid 41$) & 0.15 \\
     &  & 20.0 & 127 &  ($95 \mid 32$) & 150 &  ($109 \mid 41$) & 0.13 \\
    \cline{2-8}
     & \multirow{3}{*}{2} & 0.1 & 122 &  ($94 \mid 28$) & 158 &  ($122 \mid 36$) & \lopt{0.21} \\
     &  & 5.0 & \lopt{157} &  ($118 \mid 39$) & \lopt{183} &  ($131 \mid 52$) & 0.17 \\
     &  & 20.0 & 148 &  ($111 \mid 37$) & 177 &  ($125 \mid 52$) & 0.16 \\
    \cline{2-8}
     & \multirow{3}{*}{5} & 0.1 & 120 &  ($98 \mid 22$) & 161 &  ($127 \mid 34$) & \lopt{0.23} \\
     &  & 5.0 & 169 &  ($124 \mid 45$) & 209 &  ($146 \mid 63$) & 0.22 \\
     &  & 20.0 & \lopt{184} &  ($130 \mid 54$) & \lopt{221} &  ($146 \mid 75$) & 0.21 \\
    \bottomrule
    \end{tabular}
